What Will the Future of UAV Cellular Communications Be? A Flight from 5G to 6G

What will the future of UAV cellular communications be? In this tutorial article, we address such a compelling yet difficult question by embarking on a journey from 5G to 6G and sharing a large number of realistic case studies supported by original results. We start by overviewing the status quo on UAV communications from an industrial standpoint, providing fresh updates from the 3GPP and detailing new 5G NR features in support of aerial devices. We then show the potential and the limitations of such features. In particular, we demonstrate how sub-6 GHz massive MIMO can successfully tackle cell selection and interference challenges, we showcase encouraging mmWave coverage evaluations in both urban and suburban/rural settings, and we examine the peculiarities of direct device-to-device communications in the sky. Moving on, we sneak a peek at next-generation UAV communications, listing some of the use cases envisioned for the 2030s. We identify the most promising 6G enablers for UAV communication, those expected to take the performance and reliability to the next level. For each of these disruptive new paradigms (non-terrestrial networks, cell-free architectures, artificial intelligence, reconfigurable intelligent surfaces, and THz communications), we gauge the prospective benefits for UAVs and discuss the main technological hurdles that stand in the way. All along, we distil our numerous findings into essential takeaways, and we identify key open problems worthy of further study.

==> extra_stuff.tex <==
\vspace{2cm}

\color{lightgray}
\section*{4G LTE Support for Aerial Vehicles}

\begin{itemize}

\item Evaluation assumptions: Theory vs. simulations vs. measurements
\begin{itemize}
    \item Analytical approach for theoretical studies \cite{azari2017coexistence,AzaRosPol2019,AzaGerGar2020}; comparison of analytical modeling and frameworks; misusing of channel models.
    \item 3GPP channel modeling and simulation assumptions \cite{3GPP36777}
    \item Measurements \cite{LinWirEul2019,AmoKovWig2019,MarGuvDut2020,KovAmoNgu2017,NguAmoWig2018,HayBetFak2019}
\end{itemize}

\item{Standardized solutions in LTE-A (Rel. 15)}
\begin{itemize}
    \item New signaling for UE height and interference detection
    \item Subscription-based access against rogue UAVs
\end{itemize}

\end{itemize}

\section*{4G and 5G Use Cases and Requirements}

\begin{itemize}

\item{Background: 4G LTE use cases and requirements}

\begin{itemize}
    \item Cellular-connected UAVs for video streaming, images, other sensor data, etc. \cite{3GPP36777}.
    \item C\&C: 50 ms latency, 60-100 kbps for UL/DL, $10^{-3}$ packet loss rate \cite{3GPP36777}.
    \item Application data: latency similar to LTE UE, up to 50 Mbps for UL, no packet loss rate specified. Uplink-heavy traffic when compared to ground UE \cite{3GPP36777}.
\end{itemize}

\item{Use cases in the 2020s}

\begin{itemize}
    \item High resolution video live broadcasting
    \item Radio access through UAV
    \item Autonomous UAVs controlled by AI
    \item \emph{Create bullets for the most representative use cases in NR Rel. 17 \cite{3GPP22125,3GPP22829,AbdMar2020}.}
\end{itemize}

\item{Requirements in the 2020s}

\begin{itemize}
    \item Application data: up to 120Mbps per UAV and 20ms latency.
    \item C\&C: up to 99.99\% reliability, support of up to 300km/h.
    \item Positioning other than navigation: up to 10cm accuracy, with 99\% availability and 1s latency.
\end{itemize}

\end{itemize}

 \section*{UAV Cellular Communications Beyond 5G}
 
\begin{itemize}

\item Use cases in the 2030s
\begin{itemize}
    \item Same use cases as in 5G NR but with more UAVs; more demanding use cases with UAVs as access nodes.
    \item 3D aerial highways for goods delivery \cite{CheJaaYan2020,AmazonPrimeAir}.
    \item Flying cars to reduce congestion in megalopolis and save on fuel \cite{Saracco}. Over 100 cities working on urban air mobility solutions \cite{RolandBerger}. Market for autonomous flying cars to amount to \$1.5 trillion by 2040 \cite{Yahoo}.
\end{itemize}
    
\item Requirements in the 2030s
\begin{itemize}
\item Hyper-high data rates, lower latency achieved by sending non-compressed videos.
\item Ultra reliability, everywhere coverage in 3D environment; cm-grade localization.
\end{itemize}

\item Regulatory and security aspects \cite{stocker2017review,Yahoo}.

\end{itemize}

\color{black}
